Coin Flipping Neural Networks

We show that neural networks with access to randomness can outperform deterministic networks by using amplification. We call such networks Coin-Flipping Neural Networks, or CFNNs. We show that a CFNN can approximate the indicator of a $d$-dimensional ball to arbitrary accuracy with only 2 layers and $\mathcal{O}(1)$ neurons, where a 2-layer deterministic network was shown to require $\Omega(e^d)$ neurons, an exponential improvement (arXiv:1610.09887). We prove a highly non-trivial result, that for almost any classification problem, there exists a trivially simple network that solves it given a sufficiently powerful generator for the network's weights. Combining these results we conjecture that for most classification problems, there is a CFNN which solves them with higher accuracy or fewer neurons than any deterministic network. Finally, we verify our proofs experimentally using novel CFNN architectures on CIFAR10 and CIFAR100, reaching an improvement of 9.25\% from the baseline.

==> tex_files/experimental_study.tex <==
In this section we provide an experimental study on a set of standard image classification benchmarks: MNIST, CIFAR-10 and CIFAR-100. Our aims are 
\begin{enumerate}
    \item Observe if the CF-NN model can indeed "learn to use randomness".
    \item Examine the behaviour of CF-NN models using different \todoinline{architecture archetypes} and loss functions.
    \item Show that Coin-Flipping NNs have improved performance using the Random Accuracy metric over \todoinline{Classic Accuracy? Need to rebrand this...}
\end{enumerate}
\paragraph{Losses used}
\todoinline{TODO}
\paragraph{Comparison Method}
\todoinline{Something about Accuracy is a single-use sample from $\hat{N}(x)$, and random usage can be measured as Mean Toss Rate, $\hat{\delta}(x)$-curve or as the difference between Random Accuracy and Accuracy. Also some words about number of parameters, depth etc.}
\paragraph{MNIST}
We used the classic MNIST dataset without any filters or normalization. We used a linear base model and compared it to three models, Input RA, Output RA and Pure Random Hypernet with a linear output function. The Input and Output-RA can be said to have 2 layers, hence we also used a 2-layer linear network for comparison. No model had any non-linear activations, except a Sigmoid applied to the output of the attention network in RA models, to keep the outputs in $[0,1]$. The RA models were intialized such that the toss rate will be close to 0, to avoid over-noising that could prevent learning. The results are described in the following table:
\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 Model & Loss & Accuracy & Random Accuracy \\ [0.5ex] 
 \hline\hline
 1-Layer Linear & CEL & 90.26 & - \\ 
 \hline
 2-Layer Linear & CEL & 93.19 & - \\ 
 \hline
 Input RA & Curr + Hinge @(0.5) & 91.32 & \textbf{96.26} \\
 \hline
 Output RA \todoinline{REDO} \\
 \hline
 Pure Hyper Linear & Curr + Hinge @(0.5) & 82.91 & 92.84 \todoinline{Recalc - new definition} \\  [1ex]
 \hline
\end{tabular}
\end{center}
As can be seen in the table above, models that use randomness can both (1) achieve a higher Random Accuracy than the non-CF model with a comparable number of parameters and depth. Note that for the PHN linear model, it essentially learned an input-independent distribution on 1-layer linear functions which is 2.5\% better than the 1-layer model which directly learns the MNIST task.
We can further examine the RA models' behaviours by observing the mean of the RG's toss rate (over the entire dataset) as a function of the epoch.
\begin{figure} [h]
    \centering
    \includegraphics[scale=0.5]{figures/placeholder_first_mean_toss_rate_plot.png}
    \caption{RG Mean Toss Rate - REDO plot for Input RA}
    \label{fig:mnist_mean_toss_rate}
\end{figure}
As can be seen in \ref{fig:mnist_mean_toss_rate}, the model is initialized near 0, and as training progresses it \emph{learns to increase the randomness} of the input. This is direct evidence of the benefit the model gets from randomization.
\todoinline{This isn't very impressive - I have plots from CIFAR-100 with Toss rate above 0.6 and even 0.7, meaning the model REALLY wants to randomize... Perhaps save this plot for the CIFAR subsection?}
\par Another figure that illustrates the benefit of randomness is \ref{fig:success_rate_threshold}. In it we have three axes with a shared x-axis denoting an index of images $x$ in the dataset from 0 to 1. 
The first plot shows the difference $\hat{\delta}(x)$, i.e. the difference between the observed frequency of correct classifications from the greates frequency of any other classification. The plot is sorted in descending order of $\hat{\delta}(x)$.
Note that all inputs $x$ for which $\hat{\delta}(x) > 0$ will be correctly classified after taking $\argmax$ over a large enough $n$.
This means that the Random Accuracy of a model can be observed as the ratio of images for which $\hat{\delta}(x) > 0$, i.e. as the crossover point of the x-axis in the first plot in \ref{fig:success_rate_threshold}.
The second plot shows the values of $\hat{p}_{f(x)}$ and of 
\begin{figure} [h]
    \centering
    \includegraphics[scale=.8]{figures/placeholder_threshold_graph.png}
    \caption{Threshold - REDO for Input RA}
    \label{fig:success_rate_threshold}
\end{figure}
\paragraph{CIFAR-10 and CIFAR-100}
After showing that the model can indeed benefit from randomness, and learning can induce an increase in randomization by the model, we move on to the more challenging CIFAR-10 and CIFAR-100. 
\todoinline{Observed "bias trap" that forces a model to have outputs close to 1}
\paragraph{Input RA - linear}
\paragraph{Pure Hypernet Linear model}
\paragraph{ResNet Based Models}
base model description (a variant of a ResNet)
\paragraph{Pure Hyper Resnet}
\paragraph{Linear and ResNet attentions}
\paragraph{Input-Output Attention}
\paragraph{Dense-Random-Attention}
\begin{figure} [h]
    \centering
    \includegraphics[scale=.8]{figures/placeholder_threshold_graph.png}
    \caption{PLACEHOLDER from CIFAR100}
    \label{fig:success_rate_threshold_cifar100}
\end{figure}
\paragraph{Summary Table}
\todoinline{PLACEHOLDER}
CIFAR-100:
\begin{center}
 \begin{tabular}{||c c c c||} 
 \hline
 Model & Loss & Accuracy & Random Accuracy \\ [0.5ex] 
 \hline\hline
 2-layer ResNet & CEL & 32.02 & - \\ 
 \hline
 4-layer ResNet & CEL & 27.04 & - \\ 
 \hline
 6-layer ResNet & CEL & 21.48 & - \\ 
 \hline
 Input-Output RA & sr-largest @(.1) + o-equi & 29.61 & \textbf{39.55} \\
 \hline
 Dense RA & sr-largest @(.05) + o-equi & 29.92 & 35.81 \\  [1ex]
 \hline
\end{tabular}
\end{center}
\paragraph{Learning speed as measured in epochs}
\todoinline{I'm not certain about our reasoning for this}


\begin{comment}
\subsection{Claims}
\begin{itemize}
    \item (experimental) Random accuracy increases relative to "normal" accuracy
    \item (maybe) (proof(?) + experimental) Number of parameters decreases using RaNN (with comparable accuracy) == capacity is greater
    \item (maybe) (experimental) Learning rate is faster
    \item loss function estimation as described can be used to train
    \item Chernoff lower bound as a good loss estimation?
    \item $E[L] \rightarrow [sr > 0.5]$ as $n \rightarrow \infty$ ?
    \item hinge loss is a good substitute
    \item Show how to "tune" the network to forgo single-image accuracy for overall Random Accuracy
\end{itemize}


We have:
Models:
\begin{enumerate}
    \item Random Gate
    \begin{enumerate}
        \item Random Attention at input (and output)
    \end{enumerate}
    \item Random Hypernet
    \begin{enumerate}
        \item Pure
        \item With image as input
    \end{enumerate}
    \item Stocahstic Network (Randomized neurons)
\end{enumerate}
\begin{enumerate}
    \item MNIST "proof" that a net can learn to use random
    \begin{enumerate}
        \item Variance as a measure of "how much I want to randomize" is rising
        \item Random Accuracy can be higher than Deterministic Accuracy, by as much as 50\% (30->80)
        \item Comparison of loss functions, talk a bit about regularization
    \end{enumerate}
    \item Usefulness (on CIFAR)
    \begin{enumerate}
        \item Graph of \# Parameters vs. Random Accuracy
        \item Graph of "ratio of accuracy from final accuracy achieved" against epochs
        \item Graph of "epoch in which we got 0.95\% of final loss achieved" against \# parameters
    \end{enumerate}
\end{enumerate}

\subsection{Experiments}
\begin{enumerate}
    \item Take a trained network and validate with 1000 tries that majority gives the reported Random Accuracy
    \item Series of experiments to show that random works "on its own"
    \item Comparison between "with" and "without" random
\end{enumerate}

\begin{enumerate}
    \item Simple as possible - POC
    \begin{enumerate}
        \item Random Gate on MNIST
        \item Using a random-firing neuron
        \item Using random to decide what weights to use / randomize the weights
    \end{enumerate}
    \item Classification - CIFAR / ImageNet
    \begin{enumerate}
        \item Naively noising some internal embeddings ("Random Attention")
        \item Adding a state that is parallel to the embeddings (and used by them)
        \item Using a random-firing neuron
        \item An RNN that decides when it is ready to classify
    \end{enumerate}
    \item Adversarial examples / Adversarial learning
    \item Sequence2Seqeunce / Sequence regression
    \item Complexity-theoretic (e.g. learning to calculate discrete log)
\end{enumerate}
\end{comment}

\todoinline{https://github.com/kuangliu/pytorch-cifar - a summary of models and performance on CIFAR10 with pytorch, probably can't be used as a reference though...}
